Perceptual-based deep-learning denoiser as a defense against adversarial attacks on ASR systems

In this paper we investigate speech denoising as a defense against adversarial attacks on automatic speech recognition (ASR) systems. Adversarial attacks attempt to force misclassification by adding small perturbations to the original speech signal. We propose to counteract this by employing a neural-network based denoiser as a pre-processor in the ASR pipeline. The denoiser is independent of the downstream ASR model, and thus can be rapidly deployed in existing systems. We found that training the denoisier using a perceptually motivated loss function resulted in increased adversarial robustness without compromising ASR performance on benign samples. Our defense was evaluated (as a part of the DARPA GARD program) on the 'Kenansville' attack strategy across a range of attack strengths and speech samples. An average improvement in Word Error Rate (WER) of about 7.7% was observed over the undefended model at 20 dB signal-to-noise-ratio (SNR) attack strength.

==> abstract.tex <==
\section{Possible Titles:}

1. Perceptual Based Denoising as a Defense against Adversarial Attacks on ASR Systems 

2. Neural-Network Denoising Based Defenses Against Adversarial ASR Attacks

3. Defending Speech Recognition Systems using Neural-Network Denoising with Perceptual Loss Function

\textbf{4. Perceptual-based Deep-Learning Denoiser as a Defense Against Adversarial Attacks on ASR Systems}

\section{Preliminary Abstract:}
In this paper we investigate speech denoising as a defense against adversarial attacks on automatic speech recognition (ASR) systems. Adversarial attacks attempt to force miss-classification by adding small perturbations to the original speech signal. Ideally these perturbations are imperceptible to human listeners. We attempt to counteract this by employing a neural-network based denoiser as a pre-processor in the ASR pipeline. We found that training this denoisier using a perceptually-motivated loss function resulted in increased adversarial robustness. Our defense was evaluated on the 'Kenansville' and 'imperceptible' attack strategies across a range of attack strengths and speech samples. An average improvement in Word Error Rate (WER) of about $7.7\%$ and $xx\%$ (TBD) was observed over the undefended model under the Kenansville and imperceptible attacks, respectively, at 20 dB signal-to-noise-ratio (SNR) attack strength.  

